Mini-Batch Consistent Slot Set Encoder for Scalable Set Encoding

Most existing set encoding algorithms operate under the implicit assumption that all the set elements are accessible, and that there are ample computational and memory resources to load the set into memory during training and inference. However, both assumptions fail when the set is excessively large such that it is impossible to load all set elements into memory, or when data arrives in a stream. To tackle such practical challenges in large-scale set encoding, the general set-function constraints of permutation invariance and equivariance are not sufficient. We introduce a new property termed Mini-Batch Consistency (MBC) that is required for large scale mini-batch set encoding. Additionally, we present a scalable and efficient attention-based set encoding mechanism that is amenable to mini-batch processing of sets, and capable of updating set representations as data arrives. The proposed method adheres to the required symmetries of invariance and equivariance as well as maintaining MBC for any partition of the input set. We perform extensive experiments and show that our method is computationally efficient and results in rich set encoding representations for set-structured data.

==> figures/modelnet/deepsets_degradation.tex <==
\begin{wrapfigure}{r}{0.25\textwidth}
  \begin{center}
    \includegraphics[width=0.20\textwidth]{images/modelnet/deepsets_degradation.pdf}
  \end{center}
  \vspace{-0.2in}
  \caption{\small \label{fig:deepsets_degradation}}
\end{wrapfigure}

==> rebuttal/generalization_small.tex <==
\begin{wrapfigure}{r}{0.2\textwidth}
\centering
\vspace{-0.2in}
\includegraphics[width=0.2\textwidth]{images/celeba/generalization_small.pdf}
\vspace{-0.4in}
\caption{\small Generalization on Small Set Sizes \label{fig1}}
\vspace{-0.2in}
\end{wrapfigure}

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{in section~\ref{sec:conclusion} we discuss possible future extensions to specific limitations of our model.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We discuss this in the Appendix}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See section~\ref{sec:approach}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{see Section~\ref{sec:minibatch} and the Appendix}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{see the URL in the abstract}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{ We specify these in the Appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report results on multiple runs.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We discuss the training setup in the Appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{In the Related Work and Appendix.}
  \item Did you mention the license of the assets?
    \answerNA{Datasets are widely used open source datasets.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide a link to source code in the Abstract.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{Not applicable for our experiments.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{Not applicable for our experiments.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{Not applicable for our experiments.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{Not applicable for our experiments.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{Not applicable for our experiments.}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/modelnet/modelnet_app.tex <==
\begin{table*}
\begin{center}
  \caption{\small Test Accuracy for Point Cloud Classification with varying set sizes.\label{table:modelnet}}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{lccccc}
  \toprule
  Model             &   100                 & 200                & 500                 & 1000                & 5000                 \\
  \midrule
  DS		    &   0.8428 $\pm$ 0.0027 & 0.8518 $\pm$ 0.0032 & 0.8574 $\pm$ 0.0017 & 0.8528 $\pm$ 0.0020 & \textbf{0.8883 $\pm$ 0.0008} \\
  ST		    &   0.8258 $\pm$ 0.0042 & 0.8443 $\pm$ 0.0023 & 0.8545 $\pm$ 0.0019 & 0.8511 $\pm$ 0.0018 & 0.8604 $\pm$ 0.0009 \\
  PNA & 0.8290 $\pm$ 0.0070 & $-$ & $-$ & 0.8640 $\pm$ 0.0060 & $-$ \\
  LSTM & 0.7870 $\pm $0.0110 & $-$ & $-$ & 0.8220 $\pm$ 0.0170 & $-$ \\
  LAF & 0.8400 $\pm$ 0.0060 & $-$ & $-$ & 0.8700 $\pm$ 0.0050 & $-$ \\
  \midrule
  SSE(D)	    &   \textbf{0.8556 $\pm$ 0.0048} & 0.8633 $\pm$ 0.0038 & \textbf{0.8710 $\pm$ 0.0040} & 0.8720 $\pm$ 0.0009 & 0.8784 $\pm$ 0.0023 \\
  SSE(R)	    &   0.8532 $\pm$ 0.0009 & \textbf{0.8667 $\pm$ 0.0028} & 0.8699 $\pm$ 0.0020 & \textbf{0.8743 $\pm$ 0.0021} & 0.8853 $\pm$ 0.0012 \\
  \bottomrule
  \end{tabular}
  }
\end{center}
\end{table*}

